Few-Shot Classification of Interactive Activities of Daily Living (InteractADL)

Understanding Activities of Daily Living (ADLs) is a crucial step for different applications including assistive robots, smart homes, and healthcare. However, to date, few benchmarks and methods have focused on complex ADLs, especially those involving multi-person interactions in home environments. In this paper, we propose a new dataset and benchmark, InteractADL, for understanding complex ADLs that involve interaction between humans (and objects). Furthermore, complex ADLs occurring in home environments comprise a challenging long-tailed distribution due to the rarity of multi-person interactions, and pose fine-grained visual recognition tasks due to the presence of semantically and visually similar classes. To address these issues, we propose a novel method for fine-grained few-shot video classification called Name Tuning that enables greater semantic separability by learning optimal class name vectors. We show that Name Tuning can be combined with existing prompt tuning strategies to learn the entire input text (rather than only learning the prompt or class names) and demonstrate improved performance for few-shot classification on InteractADL and 4 other fine-grained visual classification benchmarks. For transparency and reproducibility, we release our code at https://github.com/zanedurante/vlm_benchmark.

==> old_tables/image_level.tex <==
\begin{table}[t!]

 \centering
 \resizebox{1.0\columnwidth}{!}{%
  \begin{tabular}{llccccc}
   \toprule
    Dataset &
    Method &
    1-shot &
    2-shot &
    4-shot &
    8-shot &
    16-shot \\
    
    \midrule

    Oxford Pets &
    CoOp \cite{Coop-zhou2021learning} &
    \textbf{87.1} &
    \textbf{86.4} &
    \textbf{87.8} &
    \textbf{89.6} &
    \textbf{90.1} \\

    &
    Name Tuning &
    82.7 &
    84.8 &
    86.5 &
    87.5 &
    89.0 \\

    \midrule

    Oxford Flowers &
    CoOp \cite{Coop-zhou2021learning} &
    74.9 &
    80.4 &
    86.8 &
    91.4 &
    93.6 \\

    &
    Name Tuning &
    \textbf{76.2} &
    \textbf{83.4} &
    \textbf{89.0} &
    \textbf{92.4} &
    \textbf{95.0} \\

    \midrule

    Food101 &
    CoOp \cite{Coop-zhou2021learning} &
    \textbf{79.5} &
    \textbf{79.9} &
    \textbf{80.0} &
    \textbf{81.0} &
    \textbf{81.5} \\

    &
    Name Tuning &
    75.9 &
    77.4 &
    78.7 &
    79.7 &
    80.8 \\

    \bottomrule

    \end{tabular}
}
\caption{\textbf{Name Tuning and CoOp results on few-shot image classification.} Both methods are evaluated using CLIP ViT-b32 as the pretrained VLM.}
\label{tab:image_level}
\end{table}

==> old_tables/interactadl.tex <==
\begin{table}[t!]

\centering
\resizebox{1.0\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
   \toprule
    Method &
   1-shot &
   2-shot &
   4-shot &
   8-shot \\
   
   \midrule

    Linear Probe  &
   x &
   x &
   x &
   x \\
   
   VL-Prototype  \cite{luo2022moma} &
   % no prompts
   %69.4, 58.9, 39.4 &
   %69.5, 61.3, 42.3 &
   %69.6, 64.0, 45.5 &
   %69.6, 66.6, 48.4 &
   %69.7, 68.2, 50.0 &\\

   % individual prompts
   %71.4, 59.2, 42.2 &
   %72.0, 61.3, 43.3 &
   %72.2, 64.0, 45.8 &
   %72.6, 66.4, 48.3 &
   %71.9, 67.9, 50.1 &\\

   % prompt ensemble
   x &
   x &
   x &
   x \\
    
    
   CoOp \cite{Coop-zhou2021learning} &
    x &
    x &
    x &
    x \\

    ViFi-CLIP* \cite{rasheed2023vificlip} &
    x &
    x &
    x &
    x \\

    \midrule
    Name tuning (ours) & 
    x & 
    x &
    x & 
    x \\
   
    CoNa  (ours) &
    x &
    x &
    x &
    x \\
   
    %CoN-Adapter (ours)  &
    %67.9 &
    %68.7 &
    %73.3 &
    %75.8 &
    %77.3 \\
   
   \bottomrule

  \end{tabular}
}
 \caption{\textbf{X-way few-shot classification results on the InteractADL dataset.} We obtain results using pre-trained checkpoints for CLIP, MILES, and VideoCLIP and report the highest performing backbone for each method and shot count in the table below.  See the Appendix for results on each backbone. We \textbf{bold} the highest accuracy for each  number of shots.}
     \label{tab:interactadl}

\end{table}

==> old_tables/kinetics.tex <==
\begin{table}[t!]

\centering
\resizebox{1.0\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
   \toprule
    Method &
   1-shot &
   2-shot &
   4-shot &
   8-shot &
   16-shot \\
   
   \midrule

    Prompt Engineering  &
    72.4 &
    72.4 &
    72.4 &
    72.4 &
    72.4   \\

       Linear Probe  &
   45.9 &
   55.2 &
   61.9 &
   66.8 &
   71.1 \\
   
   VL-Prototype  \cite{luo2022moma} &
   % no prompts
   %69.4, 58.9, 39.4 &
   %69.5, 61.3, 42.3 &
   %69.6, 64.0, 45.5 &
   %69.6, 66.6, 48.4 &
   %69.7, 68.2, 50.0 &\\

   % individual prompts
   %71.4, 59.2, 42.2 &
   %72.0, 61.3, 43.3 &
   %72.2, 64.0, 45.8 &
   %72.6, 66.4, 48.3 &
   %71.9, 67.9, 50.1 &\\

   % prompt ensemble
   72.2 &
   72.3 &
   72.2 &
   71.9 &
   70.9 \\
   

   
   TIP-Adapter \cite{TIPAdapter} &
    % tip-adapter no prompt ensemble
    %70.5, 59.3, 35.1 &
    %71.4, 61.5, 38.5 &
    %73.3, 63.4, 46.4 &
    %74.1, 67.7, 53.8 &
    %76.4, 69.2, 60.2 &\\

    % tip-adapter prompt ensemble
    72.2 &
    73.3 &
    74.3 &
    75.6 &
    77.3 \\
    
    
   CoOp \cite{Coop-zhou2021learning} &
    70.0 &
    72.1 &
    73.0 &
    75.3 &
    76.1 \\

    \midrule
    Name tuning (ours) & 
    \textbf{73.2} & 
    \textbf{73.8} &
    \textbf{74.7} & 
    \textbf{76.0} & 
    77.7 \\
   
    CoNa  (ours) &
    69.9 &
    71.7 &
    73.4 &
    \textbf{76.0} &
    \textbf{77.8} \\
   
    %CoN-Adapter (ours)  &
    %67.9 &
    %68.7 &
    %73.3 &
    %75.8 &
    %77.3 \\
   
   \bottomrule

  \end{tabular}
}
 \caption{\textbf{100-way few-shot classification results on the Kinetics-100 dataset.} We obtain results using pre-trained checkpoints for CLIP, MILES, and VideoCLIP and report the highest performing backbone for each method and shot count in the table below.  See the Appendix for results on each backbone. We \textbf{bold} the highest accuracy for each  number of shots.}
     %\label{tab:kinetics}

\end{table}

==> old_tables/meta-learning-kinetics.tex <==
%\begin{table*}[b]
%\resizebox{\columnwidth}{!}{
% 
 %
% \centering
% \resizebox{\columnwidth}{!}{% <------ Don't forget this %
 
%  \begin{tabular}{lc}
%  Dataset              & Average cosine similarity           \\
% \hline
%  MOMA Activities       & Val 1 \\
%  Kinetics-100          & Val 2 \\ 
%  MOMA Sub-activities   & Val 3 \\
%  SSv2                  & Val 4 \\
  %
%  \end{tabular}% <------ Don't forget this %
%}
 
 % \begin{tabular}{lc}
 %  \hline
 %  MOMA activities & 5\\
 %  \hline
 %   \label{tab:class-similarity}
% \caption{}
% \end{tabular}
% 
%}
%\end{table*}

\begin{table}[t]

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc}
\toprule
  Method              & Needs meta-train? & Accuracy        \\
 \midrule
  OTAM   \cite{otam}                            &       \checkmark     &   85.8                \\ 
  AMeFu-Net \cite{fu2020depth}                  &       \checkmark     &   86.8                       \\
  \midrule
    Linear Probe                          & \xmark            & 92.7 \\

  VL-Prototype   \cite{luo2022moma}                       & \xmark            & 93.5 \\
  TIP-Adapter \cite{TIPAdapter}         & \xmark            & 93.5 \\
  CoOp \cite{Coop-zhou2021learning}     & \xmark            & 92.7 \\
  \midrule
  Name Tuning (ours)                    & \xmark            & \textbf{94.7} \\
  CoNa (ours)                           & \xmark            & 92.0 \\


\bottomrule
\end{tabular}
}
\caption{\textbf{Comparison vs state-of-the-art meta-learning algorithms for the Kinetics-100 dataset.}  We show performance using standard 5-shot 5-way accuracy on the meta-test set. We note that the VLM-based few-shot learning approaches do not make use of the meta-train set.}
\label{tab:meta-learning-kinetics}

\end{table}

==> old_tables/meta-learning-moma-act.tex <==
%\begin{table*}[b]
%\resizebox{\columnwidth}{!}{
% 
 %
% \centering
% \resizebox{\columnwidth}{!}{% <------ Don't forget this %
 
%  \begin{tabular}{lc}
%  Dataset              & Average cosine similarity           \\
% \hline
%  MOMA Activities       & Val 1 \\
%  Kinetics-100          & Val 2 \\ 
%  MOMA Sub-activities   & Val 3 \\
%  SSv2                  & Val 4 \\
  %
%  \end{tabular}% <------ Don't forget this %
%}
 
 % \begin{tabular}{lc}
 %  \hline
 %  MOMA activities & 5\\
 %  \hline
 %   \label{tab:class-similarity}
% \caption{}
% \end{tabular}
% 
%}
%\end{table*}

\begin{table}[tb]

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc}
\toprule
  Method              & Needs meta-train? & Accuracy        \\
 \midrule
  CMN   \cite{cmn}                              &        \checkmark & 86.3            \\ 
  OTAM \cite{otam}                              &        \checkmark & 92.07                      \\
  \midrule
    Linear Probe                          & \xmark            & 96.1 \\

  VL-Prototype  \cite{luo2022moma}                        & \xmark            & 95.9 \\
  TIP-Adapter \cite{TIPAdapter}         & \xmark            & 96.0 \\
  CoOp \cite{Coop-zhou2021learning}     & \xmark            & 95.7 \\
  \midrule
  Name Tuning (ours)                    & \xmark            & \textbf{97.9} \\
  CoNa (ours)                           & \xmark            & 95.7 \\


\bottomrule
\end{tabular}
}
\caption{\textbf{Comparison vs state-of-the-art meta-learning algorithms for the MOMA Activities dataset.}  We show performance using standard 5-shot 5-way accuracy on the meta-test set. We note that the VLM-based few-shot learning approaches do not make use of the meta-train set.}
\label{tab:meta-learning-moma-act}

\end{table}

==> old_tables/meta-learning-moma-sact.tex <==
%\begin{table*}[b]
%\resizebox{\columnwidth}{!}{
% 
 %
% \centering
% \resizebox{\columnwidth}{!}{% <------ Don't forget this %
 
%  \begin{tabular}{lc}
%  Dataset              & Average cosine similarity           \\
% \hline
%  MOMA Activities       & Val 1 \\
%  Kinetics-100          & Val 2 \\ 
%  MOMA Sub-activities   & Val 3 \\
%  SSv2                  & Val 4 \\
  %
%  \end{tabular}% <------ Don't forget this %
%}
 
 % \begin{tabular}{lc}
 %  \hline
 %  MOMA activities & 5\\
 %  \hline
 %   \label{tab:class-similarity}
% \caption{}
% \end{tabular}
% 
%}
%\end{table*}

\begin{table}[htb]

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc}
\toprule
  Method              & Needs meta-train? & Accuracy        \\
 \midrule
  CMN   \cite{cmn}                              &       \checkmark & 66.6                \\ 
  OTAM \cite{otam}                              &         \checkmark & 72.6                       \\
  \midrule
    Linear Probe                          & \xmark            & 75.1 \\

  VL-Prototype   \cite{luo2022moma}                       & \xmark            & 75.7 \\
  TIP-Adapter \cite{TIPAdapter}         & \xmark            & 77.0 \\
  CoOp \cite{Coop-zhou2021learning}     & \xmark            & 76.6 \\
    \midrule
  Name Tuning (ours)                    & \xmark            & \textbf{78.2} \\
  CoNa (ours)                           & \xmark            & 76.4 \\


\bottomrule
\end{tabular}
}
\caption{\textbf{Comparison vs state-of-the-art meta-learning algorithms for the MOMA Sub-activities dataset.}  We show performance using standard 5-shot 5-way accuracy on the meta-test set. We note that the VLM-based few-shot learning approaches do not make use of the meta-train set.}
\label{tab:meta-learning-moma-sact}
\end{table}

==> old_tables/moma-act.tex <==
\begin{table}[t!]

 \centering
 \resizebox{1.0\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
   \toprule
    Method &
   1-shot &
   2-shot &
   4-shot &
   8-shot &
   16-shot \\
   
   \midrule

    Prompt Engineering  &
    81.3 & 
    81.3 &
    81.3 &
    81.3 &
    81.3 \\

    Linear Probe  &
    70.6 &
    80.6 &
    86.0 &
    90.8 &
    93.0 \\
   
   VL-Prototype  \cite{luo2022moma}&
   % no prompts
   %81.0, 76.5, 56.1 &
   %81.8, 79.8, 60.4 &
   %85.3, 84.1, 63.7 &
   %88.7, 86.7, 67.6 &
   %90.2, 88.6, 68.8 &\\

   % individual prompts
   %84.5, 74.6, 60.3 &
   %85.5, 80.7, 64.7 &
   %86.2, 85.5, 68.9 &
   %87.1, 87.0, 66.9 &
   %90.2, 89.6, 72.6 &\\

   % prompt ensemble
   85.8 &
   87.5 &
   85.5 &
   88.4 &
   90.5 \\
   

   
   TIP-Adapter \cite{TIPAdapter} &
    % tip-adapter no prompt ensemble
    %86.0, 77.6, 56.7 &
    %88.4, 80.1, 60.9 &
    %90.7, 84.0, 70.1 &
    %92.8, 85.9, 74.1 &
    %94.0, 84.3, 79.1 &\\

    % tip-adapter prompt ensemble
    88.3 &
    90.5 &
    90.0 &
    93.0 &
    93.7 \\

   
   CoOp \cite{Coop-zhou2021learning} &
    88.7 &
    90.9 &
    91.7 &
    93.6 &
    95.5 \\

    \midrule
    
    Name tuning (ours) & 
    \textbf{88.9} &
    \textbf{91.6} & 
    91.0 &
    92.7 & 
    \textbf{95.8} \\
   
    CoNa (ours)  &
    87.9 &
    91.3 &
    \textbf{92.3} &
    \textbf{94.0} &
    94.7 \\
    
%    CoN-Adapter (ours)  &
%    84.1 &
%    88.7 &
%    92.0 &
%    92.6 &
%    95.3 \\
 
   
   \bottomrule

  \end{tabular}%
}
 \caption{\textbf{19-way few-shot classification results on the MOMA-LRG, activities dataset.} We obtain results using pre-trained checkpoints for CLIP, MILES, and VideoCLIP and report the highest performing backbone for each method and shot count in the table below.  See the Appendix for results on each backbone. We \textbf{bold} the highest accuracy for each  number of shots.}
      \label{tab:moma-act}

\end{table}

==> old_tables/moma-sact.tex <==
\begin{table}[t!]
\caption{\textbf{80-way few-shot classification results on the MOMA-LRG Sub-activities dataset.} We obtain results using pre-trained checkpoints for CLIP, MILES, and VideoCLIP and report the highest performing backbone for each method and shot count in the table below.  See the Appendix for results on each backbone. We \textbf{bold} the highest accuracy for each number of shots. \vspace{-10pt}}
     \label{tab:moma-sact}
% \centering
 \resizebox{1.0\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
   \toprule
    Method &
   1-shot &
   2-shot &
   4-shot &
   8-shot &
   16-shot \\
   
   \midrule

   Prompt Engineering  &
    37.9 & 
    37.9 &
    37.9 &
    37.9 &
    37.9 \\

    Linear Probe  &
    31.0 &
    35.2 &
    38.9 &
    42.1 &
    46.1 \\
   
   VL-Prototype \cite{luo2022moma}  &
   40.0 &
   40.8 &
   41.6 &
   42.7 &
   44.3 \\
   % no prompt
   %4.4, 4.9, 6.8 &
   %5.7, 5.9, 7.5 &
   %7.6, \textbf{7.7}, 8.3 &
   %9.7, 9.6, 9.1 &
   %11.8, 11.6, 10.0 &\\

   % individual prompts
   %5.4, 5.1, 7.0 &
   %6.1, 6.4, 8.0 &
   %7.8, 8.1, 9.0 &
   %9.7, 9.5, 9.3 &
   %11.8, 12.0, 10.0 &\\

   % ensemble prompts

   

   
   TIP-Adapter \cite{TIPAdapter} &
    % Tip-Adapter no prompt-ensemble
    %\textbf{5.3}, 4.8, 5.7 &
    %6.6, 6.6, \textbf{8.0} &
    %8.2, 7.2, 9.5 &
    %11.2, 9.7, \textbf{12.8} &
    %\textbf{14.8}, 11.9, \textbf{16.6} &\\

    % Tip-Adapter Prompt-Ensemble
    39.5 &
    40.5 &
    42.5 &
    45.6 &
    48.3 \\
   
   CoOp  \cite{Coop-zhou2021learning} &
    39.4 & 
    42.9 &
    43.3 &
    45.6 &
    46.4 \\

    \midrule
    
    %CoOp (redone) &
    %--- &
    %4.8, 4.4, 5.7 &
    %5.8, 5.4, 6.8 &
    %8.1, 7.5, 8.7 &
    %10.0, 8.7, 10.9 &
    %----, 11.7, 13.2\\
    
    Name tuning (ours) & 
    39.6 & 
    41.4 &
    44.6 & 
    46.8 & 
    49.2 \\
   
    CoNa (ours)  &
    \textbf{41.9} &
    \textbf{44.2} &
    \textbf{46.5} &
    \textbf{47.5} &
    \textbf{49.7} \\
    
%    CoNAdapter (ours)  &
%    37.5 &
%    40.1 &
%    45.5 &
%    46.4 &
%    49.1 \\

    % CoNa Adapter
    %4.8, 5.1, 5.8 &
    %6.3, 5.8, 8.0 &
    %8.3, 7.7, 9.5 &
    %11.9, 10.0, 12.4 &
    %16.7, 13.1, 17.3 &\\
   
   \bottomrule

  \end{tabular}
  
}

\end{table}

==> sections/0_abstract.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/combined_fig1.png}
%     \caption{The motivation for our method: Our fine-grained visual recognition dataset InteractADL poses a challenging classification task for Pre-trained Visual Language Models (VLMs), leading to our proposal of Name Tuning, a method to provide greater semantic separation between classes with linguistically similar class names. On the left, a sample timeline of performing multiple ADLs at home in our InteractADL dataset shows two 3rd-person views provided for a video, along with annotated higher-level activity labels, temporal atomic actions, and dense spatiotemporal scene graphs. For few-shot action classification, we use VLMs that have a joint video-language embedding space and which compute similarity scores between an input video and category names. For these VLMs, we seek to use a small number of training examples to learn better class names that provide greater semantic separation and improved classification performance in fine-grained settings.}
%     \label{fig:fig1}
%     \vspace{-0.5em}
% \end{figure*}

\begin{abstract}
Recognizing human activities has recently been a central focus in video understanding for different applications. Specifically for assistive robots, smart homes, and healthcare applications, understanding Activities of Daily Living (ADLs) is crucial. However, to date, few benchmarks and methods have focused on complex ADLs, especially those involving multi-person interactions. Additionally, complex ADLs occurring in home environments comprise a challenging long tailed distribution due to the rarity of multi-person interactions, and pose fine-grained visual recognition tasks due to the presence of semantically and visually similar classes. In this paper, we propose a new dataset (denoted by InteractADL), benchmark, and few-shot method for understanding complex ADLs that involve interaction between humans (and objects). Our multi-view (ego and third-person views) dataset is annotated with human-human interactions, beyond human-object relationships considered by the prior work, as well as hierarchical activity labels. For our proposed method, we focus on Visual-language models (VLMs), which have emerged as a powerful and generalizable group of models for many downstream computer vision tasks and have shown impressive zero-shot performance on high-level visual classification datasets. However, it is relatively less understood how well these models perform on fine-grained visual recognition datasets that are comprised of semantically and visually similar classes, such as InteractADL. Focusing on the subset of visual-language models trained to learn a joint embedding space for vision and language, we show a substantial drop in performance when using these models and methods on more fine-grained datasets. We then propose a novel method, Name Tuning, to enable greater semantic separability by learning optimal class name vectors. We show that Name Tuning can be combined with existing prompt tuning strategies to learn the entire input text (rather than only learning the prompt), demonstrating improved performance for few-shot fine-grained classification. 
\end{abstract}

==> sections/9_ethics.tex <==
\section{Ethics Statement}
\label{sec:ethics}
Understanding human activities within home settings holds significant potential for advancing various smart home and healthcare applications. Nonetheless, this raises important concerns regarding the erosion of the perceived sanctity and privacy of home environments. In addressing these concerns, we identify and examine four key dimensions of trustworthiness, which align with the principles delineated in previous research (e.g.,  \cite{martinez2021ethical,haque2020illuminating}): namely, \textit{privacy}, \textit{fairness}, \textit{transparency}, and \textit{research ethics}. The practical deployment of such technologies necessitates the development of a robust framework that adequately addresses these four pillars, ensuring the ethical and responsible use of artificial intelligence and computer vision technologies in home environments.
